Weighted Programming

We study weighted programming, a programming paradigm for specifying mathematical models. More specifically, the weighted programs we investigate are like usual imperative programs with two additional features: (1) nondeterministic branching and (2) weighting execution traces. Weights can be numbers but also other objects like words from an alphabet, polynomials, formal power series, or cardinal numbers. We argue that weighted programming as a paradigm can be used to specify mathematical models beyond probability distributions (as is done in probabilistic programming). We develop weakest-precondition- and weakest-liberal-precondition-style calculi \`{a} la Dijkstra for reasoning about mathematical models specified by weighted programs. We present several case studies. For instance, we use weighted programming to model the ski rental problem - an optimization problem. We model not only the optimization problem itself, but also the best deterministic online algorithm for solving this problem as weighted programs. By means of weakest-precondition-style reasoning, we can determine the competitive ratio of the online algorithm on source code level.

==> sections/2-cheat-sheet-vertical.tex <==
% !TEX root = ../weighted-programs-oopsla22.tex

\begin{table}
    \centering
	\caption{Weighted programming cheat sheet.}
	\label{fig:module-overview}
	\renewcommand{\arraystretch}{2}
	\setlength{\tabcolsep}{0.5em}
	\begin{adjustbox}{max width=1\textwidth,max height=0.96\textheight}
	\begin{sideways}
	\begin{tabular}{l l c c l l l}
		\toprule
		%
		\textbf{Weighting $\boldsymbol{\WEIGH{a}}$} & \textbf{Branching $\boldsymbol{\BRANCH{C_1}{C_2}}$} & \textbf{Application areas} & \textbf{Semiring / Module} & \makecell[c]{\textbf{Interpretation of}\\ \textbf{postweighting $\boldsymbol{f}$}} & \makecell[c]{\textbf{Interpretation of}\\ \textbf{$\boldsymbol{\wp{C}{f}}$}} & \makecell[c]{\textbf{Interpretation of}\\ \makecell[c]{\textbf{$\boldsymbol{\wlp{C}{f}}$}}}\\
		%
		\midrule
		%
		%
		\makecell[l]{Accumulate cost $a$} 
		& 
		\makecell[l]{Choose branch that will\\ accumulate \emph{minimal} cost} 
		& 
		\makecell[c]{Optimization} 
		& 
		\makecell[c]{\emph{Tropical semiring}\\[.5ex] $(\NatsInf,\, {\min},\, {+},\, {+\infty},\, 0)$}
		&
		\makecell[l]{Cost that is accumulated\\ after program termination;\\ typically choose $f = 0$} 
		&
		\makecell[l]{Minimal accumulated cost\\ amongst all terminating\\ executions of $C$, for $f=0$}  
		&
		\makecell[l]{Minimum of $\wp{C}{f}$ and \\ the minimal accumulated cost\\ amongst all non-terminating\\ executions of $C$}
		%
		\\[2ex]
		%
		%
		\midrule
		%
		%
		\makecell[l]{Accumulate cost $a$} 
		& 
		\makecell[l]{Choose branch that will\\ accumulate \emph{maximal} cost} 
		& 
		\makecell[c]{Optimization}  
		& 
		\makecell[c]{\emph{Arctic semiring} \\[.5ex] $(\NatsInf_{-\infty},\, {\max},\, {+},\, {-\infty},\, 0)$}  
		&
		\makecell[l]{Cost that is accumulated\\ after program termination;\\ typically choose $f = 0$} 
		&
		\makecell[l]{Maximal accumulated cost\\ amongst all terminating\\ executions of $C$, for $f=0$}  
		&
		\makecell[l]{Same as $\wp{C}{f}$ if all \\ executions of $C$ terminate, \\ else $+\infty$}
		%
		\\[2ex]
		%
		%
		\midrule
		%
		%
		\makecell[l]{Restrict capacity of \\ current branch to $a$} 
		& 
		\makecell[l]{Choose branch with\\ \emph{maximal} capacity} 
		& 
		\makecell[c]{Optimization}
		& 
		\makecell[c]{\emph{Bottleneck semiring}\tablefootnote{Also known as \emph{max-min-semiring}. The name \emph{Bottleneck semiring} is taken from \cite{semirings-for-breakfast}. Quantitative verification using this semiring is further studied in \cite{quantitative-strongest-post-arxiv,quantitative-strongest-post-oopsla}.} \\[.5ex] $(\Reals_{-\infty}^{+\infty},\, {\max},\, {\min},\, {-\infty},\, {+\infty})$}
		&
		\makecell[l]{Upper bound after \\ program termination; \\ typically choose $f = +\infty$}
		&
		\makecell[l]{Maximum bottleneck \\ amongst all terminating \\ executions of $C$}
		&
		\makecell[l]{Maximum bottleneck \\ amongst all executions of $C$}
		%
		\\[2ex]
		%
		%
		\midrule
		%
		%
		\makecell[l]{Append symbol $a$\\to current trace} 
		& 
		\makecell[l]{Account for/aggregate \\ behavior of both branches} 
		& 
		\makecell[c]{Model checking} 
		& 
		\makecell[c]{\emph{Formal languages} \\[.5ex] $\bigl(2^{\ab^*},\, {\cup},\, \,{\langConcat}\,,\, \emptyset,\, \set{\varepsilon}\bigr)$}  
		&
		\makecell[l]{Language that is appended\\ to each terminated trace;\\typically choose $f = \{\varepsilon\}$} 
		&
		\makecell[l]{Language of all terminating\\ traces of $C$, for $f = \{\varepsilon\}$}  
		&
		\makecell[l]{Language of all terminating\\ and nonterminating\\ traces of $C$, for $f = \{\varepsilon\}$}
		%
		\\[2ex]
		%
		%
		\midrule
		%
		%
		\makecell[l]{Make $a$ copies of\\ current path/trace} 
		& 
		\makecell[l]{Sum up number of\\ paths/traces of\\ both branches}
		& 
		\makecell[c]{Combinatorics} 
		& 
		\makecell[c]{\emph{(Extended)} \emph{natural numbers} \\[.5ex] $(\NatsInf,\, {+},\, \,{\cdot}\,,\, 0,\, 1)$}  
		&
		\makecell[l]{Number of copies that is\\ made of each terminated\\ path/trace;\\ typically choose $f = 1$} 
		&
		\makecell[l]{Number of all terminating\\ paths/traces of $C$, for $f = 1$}  
		&
		\makecell[l]{Same as $\wp{C}{f}$ if all \\ executions of $C$ terminate, \\ else $+\infty$}
		%
		\\[2ex]
		%
		%
		\midrule
		%
		%
		\makecell[l]{Let what follows \\ happen with\\ probability $a$} 
		& 
		\makecell[l]{Choose branch of  \\ maximal probability} 
		& 
		\makecell[c]{Hidden Markov \\ models} 
		& 
		\makecell[c]{\emph{Viterbi semiring} \\[.5ex] $([0,1],\, {\max},\, \,{\cdot}\,,\, 0,\, 1)$}  
		&
		\makecell[l]{Probability additionally \\ multiplied to each \\ terminated trace; \\ typically choose $f = \iverson{\varphi}$,\\i.e.\ the indicator function\\ of some event $\varphi$} 
		&
		\makecell[l]{Maximal probability of a \\ terminating execution \\ establishing $\varphi$, for $f = \iverson{\varphi}$}  
		&
		\makecell[l]{Maximal probability of a \\ non-terminating execution, \\ or a terminating execution \\ establishing $\varphi$, for $f = \iverson{\varphi}$}
		%
		\\[2ex]
		%
		%
		\midrule
		%
		%
		\makecell[l]{Assert predicate $a$} 
		& 
		\makecell[l]{Angelic choice:\\ choose \enquote{most true} branch} 
		& 
		\makecell[c]{Verification /\\ Debugging} 
		& 
		\makecell[c]{\emph{Boolean semiring} \\[.5ex] $(\{0,1\},\, {\lor},\, {\land},\, 0,\, 1)$}  
		&
		\makecell[l]{$f$ -- a predicate -- is a\\ postcondition that should\\ be established after\\ program termination.} 
		&
		\makecell[l]{Weakest precondition of $f$,\\ the weakest predicate $g$ so that\\ starting in $g$, program $C$ can\\ terminate in state $\tau \models f$}  
		&
		\makecell[l]{Weakest liberal precondition of $f$,\\ the weakest predicate $g$ so that\\ starting in $g$, program $C$ can\\ either diverge or\\ terminate in state $\tau \models f$}
		%
		\\[2ex]
		%
		%
		\midrule
		%
		%
		\makecell[l]{Use resource $a$} 
		& 
		\makecell[l]{Alternatives: use resources\\ via $C_1$ or via $C_2$}
		& 
		\makecell[c]{Feature selection} 
		& 
		\makecell[c]{\emph{Why semiring}, cf. \cite{DBLP:journals/corr/abs-1910-07910} \\[.5ex] $(\text{propositional \emph{positive} DNF}, {\lor}, {\land}, 0, 1)$ \\ over a finite set of variables $X_1, \ldots, X_n$ }
		&
		\makecell[l]{Combinations of resources \\ used after termination; \\ typically choose $f = \iverson{\varphi}$} 
		&
		\makecell[l]{Possible alternatives (disjunction) \\ of resource sets (conjunction) \\ to reach event $\varphi$, for $f = \iverson{\varphi}$}
		&
		\makecell[l]{Possible alternatives (disjunction) \\ of resource sets (conjunction) \\ to either not terminate or \\ reach event $\varphi$, for $f = \iverson{\varphi}$} \\
		%
		%
		\bottomrule
	\end{tabular}
	\end{sideways}
	\end{adjustbox}
\end{table}



==> sections/6-ski-rental-verification.tex <==
% !TEX root = ../weighted-programs-oopsla22.tex

\begin{figure}
	%
	\begin{adjustbox}{max height=65mm}
		\centering
		\begin{minipage}{0.45\textwidth}
			\begin{align*}
				& \eqannotate{\varvaclen \sadd \varbuycost \gray{\eeq I}} \\
				%
				%
				%
				&\phiannotate{\iverson{\varvaclen = 0}\ivop \sone
					\ssadd  \iverson{\varvaclen > 0}\ivop (\varvaclen 
					\sadd
					\varbuycost) 
				} \\
				%
				&\WHILE{\varvaclen > 0} \\
				%
				& \qquad \eqannotate{\varvaclen 
					\sadd
					\varbuycost
				} \\
				%
				& \qquad \wpannotate{1 \smul (\varvaclen - 1)
					\ssadd
					\varbuycost
				} \\
				%
				& \qquad \ASSIGN{\varvaclen}{\varvaclen - 1}\fatsemi \\
				%
				& \qquad \eqannotate{1 \smul \varvaclen
					\ssadd
					\varbuycost
				} \\
				%
				%
				& \qquad \wpannotate{1 \smul (\varvaclen \sadd \varbuycost)
					\ssadd
					\varbuycost
				} \\
				%
				& \qquad \{ ~ \textnormal{\textcolor{gray}{(* rent *)}}  \\
				%
				& \qquad \qquad \wpannotate{1 \smul (\varvaclen \sadd \varbuycost)} \\
				%
				&\qquad \qquad \WEIGH{1} \\
				%
				& \qquad \qquad \annotate{\varvaclen \sadd \varbuycost} \\
				%
				&\qquad \} \BranchSymbol \{  ~ \textnormal{\textcolor{gray}{(* buy *)}} \\
				%
				& \qquad \qquad \eqannotate{\varbuycost } \\
				%
				& \qquad \qquad \wpannotate{\varbuycost \smul \sone} \\
				%
				& \qquad \qquad \WEIGH{\varbuycost} \fatsemi \\
				%
				& \qquad \qquad \eqannotate{\sone} \\
				%
				& \qquad \qquad \eqannotate{0} \\
				%
				& \qquad \qquad \wpannotate{0 \sadd \varbuycost} \\
				%
				&\qquad \qquad \ASSIGN{\varvaclen}{0}  ~ \textnormal{\textcolor{gray}{(* terminate *)}}\\
				%
				& \qquad \qquad \annotate{\varvaclen \sadd \varbuycost} \\
				%
				&\qquad \} \\
				%
				& \qquad \starannotate{\varvaclen \sadd \varbuycost \gray{\eeq I}} \\
				& \} \\
				%
				& \annotate{\sone}
			\end{align*}
		\end{minipage}
		\qquad\qquad
		\begin{minipage}{0.45\textwidth}
			\begin{align*}
				&\wpannotate{\scriptstyle \iverson{\varvaclen=0} \ivop 0     \mmadd \iverson{0< \varbuycost}\ivop 
					\big( (2\varbuycost  -1) \sadd \iverson{\varvaclen \leq \varbuycost - 1}\ivop \varvaclen \big) 
				} \\
			   %
				&\ASSIGN{\varvaccount}{0}\fatsemi \\
				%
				&  \eqannotate{\scriptstyle \iverson{\varvaclen = 0} \ivop 0 \mmadd  \iverson{\varvaccount  \geq \varbuycost} \ivop \varbuycost  \mmadd  \iverson{\varvaccount  < \varbuycost} }   \\
				% 
				&\qquad \quad \quad     \phantannotate{\scriptstyle \ivop
					\big( (2\varbuycost - \varvaccount -1) \mmadd \iverson{\varvaclen \leq \varbuycost - \varvaccount - 1}\ivop \varvaclen \big)  \gray{\eeq I} } \\
				%
                 &  \phiannotate{\scriptstyle \iverson{\varvaclen = 0} \ivop 0 \mmadd \iverson{\varvaclen >0} \ivop \big(  \iverson{\varvaccount +1 \geq \varbuycost} \ivop \varbuycost  \mmadd  \iverson{\varvaccount +1 < \varbuycost} }   \\
                 % 
                 &\qquad \quad \quad     \phantannotate{\scriptstyle \ivop 
                 	\big( (2\varbuycost - \varvaccount -1) \mmadd \iverson{\varvaclen \leq \varbuycost - \varvaccount - 1}\ivop \varvaclen \big) \big) } \\
				%
				&\WHILE{\varvaclen > 0} \\
				%
				%
				%
				& \qquad \eqannotate{\scriptstyle  \iverson{\varvaccount+1 \geq \varbuycost} \ivop \varbuycost  \mmadd  \iverson{\varvaccount+1 < \varbuycost} }   \\
				% 
				&\qquad \quad \quad     \phantannotate{\scriptstyle \ivop \big(  
					 (2\varbuycost - \varvaccount -1) \mmadd \iverson{\varvaclen \leq \varbuycost - \varvaccount - 1}\ivop\varvaclen \big)  } \\
				%
				& \qquad \wpannotate{\scriptstyle \iverson{\varvaccount+1 < \varbuycost} \ivop (1 \smul I\subst{\varvaccount}{\varvaccount+1}\subst{n}{n-1}) \mmadd \iverson{\varvaccount+1 \geq \varbuycost} \ivop \varbuycost }  \\
				%
				& \qquad \ASSIGN{\varvaclen}{\varvaclen - 1}\fatsemi \\
				%
				& \qquad \wpannotate{\scriptstyle \iverson{\varvaccount+1 < \varbuycost} \ivop (1 \smul I\subst{\varvaccount}{\varvaccount+1}) \mmadd \iverson{\varvaccount+1 \geq \varbuycost} \ivop \varbuycost }  \\
				%
				& \qquad \ASSIGN{\varvaccount}{\varvaccount + 1}\fatsemi \\
				%
				& \qquad \wpannotate{\scriptstyle \iverson{\varvaccount < \varbuycost} \ivop(1 \smul I) \mmadd \iverson{\varvaccount \geq \varbuycost} \ivop \varbuycost }  \\
				%
				& \qquad \IF{\varvaccount < \varbuycost} \\
				%
				& \qquad \wpannotate{\scriptstyle 1 \smul I	} \\
				%
				& \qquad \qquad \WEIGH{1} \\
				%
				& \qquad \annotate{\scriptstyle I	} \\
				%
				& \qquad \ELSE \\
				%
				& \qquad \eqannotate{\scriptstyle \varbuycost} \\
				%
				& \qquad \wpannotate{\scriptstyle \varbuycost \smul 0} \\
				%
				& \qquad \qquad \WEIGH{\varbuycost}\fatsemi \\
				%
				& \qquad \eqannotate{\scriptstyle 0} \\
				%
				%
				& \qquad \wpannotate{\scriptstyle I\subst{n}{0}} \\
				%
				&\qquad \qquad \ASSIGN{\varvaclen}{0} \\
				%
				& \qquad \annotate{\scriptstyle I} \\
				%
				& \qquad \} \\
				%
				& \qquad \starannotate{\scriptstyle \iverson{\varvaclen=0} \ivop 0 \mmadd \iverson{\varvaccount \geq \varbuycost}\ivop \varbuycost } \\
				&\qquad \quad     \phantannotate{\scriptstyle   \mmadd \iverson{\varvaccount < \varbuycost}\ivop
					\big( (2\varbuycost - \varvaccount -1) \mmadd \iverson{\varvaclen \leq \varbuycost - \varvaccount - 1}\ivop \varvaclen \big) \gray{\eeq I}
				} \\
				%
				& \} \\
				%
				& \annotate{\scriptsize \sone}
			\end{align*}
			%
		\end{minipage}
	\end{adjustbox}
	%
	\caption{Program $\crentnondet$ (left) modeling the \emph{optimal} solution the Ski Rental Problem and program $\crentonline$ (right) implementing the optimal \emph{deterministic online} algorithm (cf.\ \cref{sec:app_ski_rental}) for all annotations.}
	\label{fig:ski_rental_programs_verification}
\end{figure}

